An Information Theoretic Framework For Designing Information Elicitation Mechanisms That Reward Truth-telling

In the setting where information cannot be verified, we propose a simple yet powerful information theoretical framework---the Mutual Information Paradigm---for information elicitation mechanisms. Our framework pays every agent a measure of mutual information between her signal and a peer's signal. We require that the mutual information measurement has the key property that any "data processing" on the two random variables will decrease the mutual information between them. We identify such information measures that generalize Shannon mutual information. Our Mutual Information Paradigm overcomes the two main challenges in information elicitation without verification: (1) how to incentivize effort and avoid agents colluding to report random or identical responses (2) how to motivate agents who believe they are in the minority to report truthfully. Aided by the information measures we found, (1) we use the paradigm to design a family of novel mechanisms where truth-telling is a dominant strategy and any other strategy will decrease every agent's expected payment (in the multi-question, detail free, minimal setting where the number of questions is large); (2) we show the versatility of our framework by providing a unified theoretical understanding of existing mechanisms---Peer Prediction [Miller 2005], Bayesian Truth Serum [Prelec 2004], and Dasgupta and Ghosh [2013]---by mapping them into our framework such that theoretical results of those existing mechanisms can be reconstructed easily. We also give an impossibility result which illustrates, in a certain sense, the the optimality of our framework.

==> extend.tex <==
\paragraph{Extended $\IMM$ ($\EIMM$($MI$))} Given setting $(n,\Sigma)$, a space $A$ and a finite set of random functions $\{g_{\ell},h_{\ell}:\Sigma^{n-1}\mapsto A\}_{\ell\in L}$ whose randomnesses are independent with the $n$ agents' private information.
\begin{description}
\item[Report] For each agent $i$, she is asked to provide her private information $\Psi_i$. We denote the actual information she reports as $\hat{\Psi}_i$. 
\item[Payment/Information Score] Excluding agent $i$, we denote the rest of agents' reports by $\hat{\Psi}_{-i}$. Agent $i$ is paid by her information score $$\sum_{\ell} MI(\hat{\Psi}_i;g_{\ell}(\hat{\Psi}_{-i})|h_{\ell}(\hat{\Psi}_{-i}))$$ where $MI$ is information-monotone. 
\end{description}

With similar proof in proving Theorem~\ref{thm:imm}, we can obtain the below theorem. 

\begin{theorem}
Extended $\imm$ $\EIMM$($MI$) is dominantly $\truthful$ when $MI$ is information-monotone.
%Extended $\imm$ $\EIMM$($MI$) has the just desserts and is dominantly $\info$ when $MI$ is information-monotone. 
\end{theorem}

Without any restrictions for the random functions $\{g_{\ell},h_{\ell}:\Sigma^{n-1}\mapsto A\}_{\ell\in L}$, it is impossible to discuss the strictness property here. We suggest analyzing the requirements of strictness property specifically when applying $\EIMM$ into concrete cases. 

\yk{The above paragraph is a little bit weird too.}


With similar proof in proving Theorem~\ref{thm:imm2}, we can obtain the below theorem. 
\begin{theorem}
%Extended $\imm$ $\EIMM$($MI$) is dominantly $\truthful$ when $MI$ is convex and information-monotone.
With assumption~\ref{assume:effort}, the Extended $\imm$ $\EIMM$($MI$) has the just desserts and is dominantly $\info$ when $MI$ is convex and information-monotone. 
\end{theorem}

==> recommend.tex <==
\begin{figure}
	\centering
	\includegraphics[width=0.9\linewidth]{order}
	\caption{Reading guide}
	\label{fig:order}
\end{figure}


We have now finished the introduction for our basic framework. 
Curious readers who are interested in the direct application of our framework can read Section~\ref{sec:md}. 
Readers who are familiar with \citet{dasgupta2013crowdsourced} may enjoy reading Section~\ref{sec:reprovemd} to see how to recast \citet{dasgupta2013crowdsourced} into our framework. Readers who are familiar with \citet{prelec2004bayesian} may enjoy reading Section~\ref{sec:bts} to see how to recast \citet{prelec2004bayesian} into our framework. Figure~\ref{fig:order} shows the perquisite sections the reader should read before they read a section of interest.


\begin{comment}


The readers now do not need to read the paper in order. The below guides are parallel to each other. 


A direct application of our framework---$f$-mutual information mechanism (Section~\ref{sec:md})---can be read directly with skipping the zero-one effort model equilibrium goals (e.g. dominantly informative) in the statement of Theorem~\ref{thm:fmutual}, after reading the backgrounds of multiple-questions setting in Section~\ref{sec:multi}.  

Section~\ref{sec:reprovemd} shows how to recast \citet{dasgupta2013crowdsourced} into a special case of $f$-mutual information and can be read after reading the definition of $f$-mutual information mechanism (Section~\ref{sec:md}) in and the backgrounds of multiple-questions setting in Section~\ref{sec:multi}. 

Section~\ref{sec:reprovepp} shows how to understand the original peer prediction method~\citet{MRZ05} using our framework and can be read after reading the backgrounds of single-question setting in Section~\ref{sec:single} and the idea of ``expected accuracy gain = information gain'' in Section~\ref{sec:bregmanmutual}.

Section~\ref{sec:bts} also uses the idea of ``expected accuracy gain = information gain'' in Section~\ref{sec:bregmanmutual} to recast the Bayesian truth serum into our framework and can be read after reading the backgrounds of single-question setting in Section~\ref{sec:single} and Section~\ref{sec:bregmanmutual}.

Section~\ref{sec:bregman} introduces a new mutual information measurements---Bregman mutual information---that preserves most of the information-monotone properties $f$-mutual information has. By plugging Bregman mutual information into our framework, the $\imm$ is not focal but still dominantly truthful. Section~\ref{sec:bregman} also provides a novel connection between log scoring rule and Shannon mutual information. A powerful application of this connection is the information theoretic reconstruction of \citet{prelec2004bayesian} (Section~\ref{sec:reprovebts}). 


Section~\ref{sec:effort} extends our framework to the setting where agents need to invest a certain amount of effort to receive their private information. 

Section~\ref{sec:impossibility} shows the impossibility results that implies that truth-telling cannot beat other $\full$ strategy when the mechanism is detail free. 

\end{comment}
